Near-Optimal $\Phi$-Regret Learning in Extensive-Form Games

In this paper, we establish efficient and uncoupled learning dynamics so that, when employed by all players in multiplayer perfect-recall imperfect-information extensive-form games, the trigger regret of each player grows as $O(\log T)$ after $T$ repetitions of play. This improves exponentially over the prior best known trigger-regret bound of $O(T^{1/4})$, and settles a recent open question by Bai et al. (2022). As an immediate consequence, we guarantee convergence to the set of extensive-form correlated equilibria and coarse correlated equilibria at a near-optimal rate of $\frac{\log T}{T}$. Building on prior work, at the heart of our construction lies a more general result regarding fixed points deriving from rational functions with polynomial degree, a property that we establish for the fixed points of (coarse) trigger deviation functions. Moreover, our construction leverages a refined regret circuit for the convex hull, which -- unlike prior guarantees -- preserves the RVU property introduced by Syrgkanis et al. (NIPS, 2015); this observation has an independent interest in establishing near-optimal regret under learning dynamics based on a CFR-type decomposition of the regret.

==> figs/tikzmacros.tex <==
\usepackage{tikz}

\usetikzlibrary{fit,shapes.misc,arrows.meta}
\makeatletter
\tikzset{
  fitting node/.style={
    inner sep=0pt,
    fill=none,
    draw=none,
    reset transform,
    fit={(\pgf@pathminx,\pgf@pathminy) (\pgf@pathmaxx,\pgf@pathmaxy)}
  },
  reset transform/.code={\pgftransformreset}
}
\tikzset{cross/.style={path picture={
  \draw[black]
(path picture bounding box.south east) -- (path picture bounding box.north west) (path picture bounding box.south west) -- (path picture bounding box.north east);
}}}
\tikzstyle{ox}=[semithick,draw=black,circle,cross,inner sep=1.2mm]

==> text/abstract.tex <==
$\Phi$-regret is a general performance metric in online learning that strengthens the standard notion of (external) regret by measuring the performance of the learner based on the optimal in hindsight deviation from $\Phi$. From a game-theoretic standpoint, the importance of this framework stems from the celebrated fact that no-$\Phi$-regret learners in games are known to converge to different \emph{correlated equilibrium} concepts, depending on the richness of the deviations included in $\Phi$. In particular, the rate of convergence is driven by the maximum $\Phi$-regret incurred by a player. Despite rapid recent progress on special cases of this problem, a central question still stands: What are the best possible guarantees when $\Phi$-regret learners are competing against each other? 
    
In this paper, we address this question by developing a general framework that enables us to establish near-optimal $\Phi$-regret guarantees under broad and natural assumptions on the set of deviations $\Phi$. As the main application of our framework, we establish efficient and uncoupled learning dynamics so that, when employed by all players in a multiplayer imperfect-information extensive-form game, the \emph{trigger regret} of each player after $T$ repetitions grows as $O(\log T)$, thereby guaranteeing convergence to the set of \emph{extensive-form correlated equilibria} at a near-optimal rate of $\frac{\log T}{T}$. This improves exponentially over the prior best known trigger-regret bound of $O(T^{1/4})$, and settles a recent open question by~Bai et al. (2022).

==> text/introduction.tex <==
\section{Introduction}
\label{section:introduction}

A primary objective of artificial intelligence (AI) is the design of agents that can adapt effectively in complex multiagent environments---modeled as \emph{general-sum games}. Multiagent decision making often occurs in a decentralized fashion, with every agent only obtaining information about its own reward function, and the goal is to \emph{learn} how to play the game through repeated interactions. This begs the question: \emph{How do we measure the performance of a learning agent?} A popular metric commonly used in the literature is that of \emph{external regret} (or simply regret). However, external regret can be a rather weak benchmark: a no-external-regret agent could still incur substantial regret under simple in-hindsight ``transformations'' of its behavior---\emph{e.g.}, consistently switching from an action $a$ to a different action $a'$~\citep{Gordon08:No}.

A more general metric is \emph{$\Phi$ regret}~\citep{Hazan07:Computational,Rakhlin11:Online,Stoltz07:Learning,Greenwald03:A}, parameterized by a set deviations $\Phi$. From a game-theoretic standpoint, the importance of this framework is that different choices of $\Phi$ lead to different types of equilibria~\citep{Greenwald03:A,Stoltz07:Learning}. One such celebrated result guarantees that \emph{no-internal-regret} players converge---in terms of empirical frequency of play---to the set of \emph{correlated equilibria (CE)}~\citep{Foster97:Calibrated,Hart00:Simple}. This brings us to the central question of our paper:
%
\begin{quote}
    \centering
    \emph{What are the best performance guarantees when no-$\Phi$-regret learners are competing in multiplayer general-sum games?}
\end{quote}
%
Special cases of this question have recently received considerably attention in the literature (see \Cref{sec:related}). In particular, \citet{Daskalakis21:Near} were the first to establish $O(\polylog(T))$ external regret bounds for normal-form games,\footnote{With a slight abuse of notation, we use the $O(\cdot)$ notation in our introduction to suppress parameters that depend (polynomially) on the description of the game.} and subsequent work extended those results to internal regret~\citep{Anagnostides21:Near}; those guarantees, applicable when \emph{all} players employ specific learning dynamics, improve exponentially over what is possible when a player is facing a sequence of adversarially produced utilities---the canonical consideration in online learning. However, much less is known about $\Phi$-regret learning beyond normal-form games. One such important application revolves around learning dynamics for \emph{extensive-form correlated equilibria (EFCE)}~\citep{Stengel08:Extensive,Gordon08:No,Celli20:No-Regret,Morrill21:Efficient,Anagnostides22:Faster,Morrill21:Hindsight,Bai22:Efficient,Song22:Sample}. Indeed, a particular instantiation of $\Phi$ regret, referred to as \emph{trigger regret}, is known to drive the rate of convergence of learning dynamics to EFCE. In this context, prior work established $O(T^{1/4})$ per-player trigger regret bounds~\citep{Anagnostides22:Faster}, thereby leaving open the possibility of obtaining near-optimal rates for EFCE; that question was also recently posed by~\citet{Bai22:Efficient}.

\subsection{Our Contributions}

Our main contribution is to develop a new framework for obtaining near-optimal $\Phi$-regret guarantees through the use of efficient and uncoupled learning dynamics in general multiplayer games. Taking a step back, the problem of minimizing $\Phi$-regret can be overly complex and computationally intractable when no structure is imposed on the set $\Phi$, necessitating further assumptions to ensure that the problem is, at the very least, tractable. In this context, our first assumption postulates efficient implementation of a \emph{proximal oracle} for $\Phi$---roughly speaking, a projection (\Cref{assumption:efficiency}). Our next key assumption is about the behavior of the \emph{fixed points} of transformations $\phi \in \Phi$; such fixed points are at the heart of the general $\Phi$-regret minimizer of~\citet{Gordon08:No}, which is also used in our work. For our purposes, we assume that the fixed points can be expressed as combinations of rational functions with a polynomial degree (\Cref{assumption:rational}). Under those conditions, we show the following.

\begin{theorem}[Informal; Precise Version in \Cref{theorem:main}]
    \label{theorem:informal}
    Under a broad class of deviations $\Phi$, there exist uncoupled and efficient learning dynamics so that the $\Phi$ regret of each player grows as $O(\log T)$ after $T$ repetitions.
\end{theorem}

Our construction instantiates the template of~\citet{Gordon08:No} with the recent algorithm of~\citet{Farina22:Near} for performing external-regret minimization over general convex sets. The importance of a rational function characterization is that it allows us to convert the \emph{RVU property}---\emph{regret bounded by variation in utilities}~\citep{Syrgkanis15:Fast}---from the space of deviations $\Phi$ to the actual space of the player's strategies. This analysis builds on a technique developed for obtaining $O(\log T)$ swap regret in normal-form games~\citep{Anagnostides22:Uncoupled}. 

As the main application of our framework, we obtain the first near-optimal guarantees for \emph{trigger regret} in extensive-form games, thereby improving exponentially over the $O(T^{1/4})$ bounds obtained in prior work~\citep{Celli20:No-Regret,Anagnostides22:Faster}:

\begin{corollary}
    There exist uncoupled and efficient learning dynamics so that the trigger regret of each player grows as $O(\log T)$ after $T$ repetitions.
\end{corollary}

This settles an open question recently posed by~\citet{Bai22:Near}, and implies the first near-optimal rates of convergence to the set of EFCE.

\begin{corollary}
    There exist uncoupled learning dynamics converging to EFCE at a near-optimal rate of $O(\frac{\log T}{T})$.
\end{corollary}

Finally, we also obtain improved rates for extensive-form \emph{coarse} correlated equilibria (EFCCE)~\citep{Farina20:Coarse}, a relaxation of EFCE that is attractive due to its reduced per-iteration complexity compared to EFCE~\citep{Anagnostides22:Faster}.

\subsection{Further Related Work}
\label{sec:related}

$\Phi$ regret has received extensive attention as a solution concept in the literature since it strengthens and unifies many common measures of performance in online learning (\emph{e.g.}, see ~\citep{Hazan07:Computational,Rakhlin11:Online,Stoltz07:Learning,Greenwald03:A,Marks08:No,Piliouras22:Evolutionary}). This framework has been particularly influential in game theory, where no-$\Phi$-regret learning outcomes are known to converge to different equilibrium concepts, depending on the richness of the set of deviations $\Phi$. For example, when $\Phi$ includes \emph{all constant transformations}---reducing to external regret---no-regret learning outcomes are known to converge to \emph{coarse correlated equilibria (CCE)}~\citep{Moulin78:Strategically}, a relaxation of CE. Unfortunately, CCE is understood to be a weak equilibrium concept, potentially prescribing irrational behavior~\citep{Dekel90:Rational,Viossat13:No,Giannou21:Survival}. This motivates enlarging the set of deviaitons $\Phi$, thereby leading to stronger---and arguably more plausible---equilibrium concepts. Indeed, the framework of $\Phi$ regret has been central in the development of the first uncoupled no-regret learning dynamics for EFCE~\citep{Celli20:No-Regret,Farina21:Simple} (see also~\citep{Morrill21:Efficient,Morrill21:Hindsight,Zhang22:A}).\footnote{While there are other methods for efficiently computing EFCE~\citep{Dudik09:SamplingBased,Huang08:Computing}, approaches based on uncoupled no-regret learning typically scale significantly better in large games.}

Our paper lies at the interface of the aforedescribed literature with a recent line of work that strives for improved regret guarantees when specific learning dynamics are in place; this allows circumventing the notorious $\Omega(\sqrt{T})$ lower bounds applicable under an adversarial sequence of utilities~\citep{Cesa-Bianchi06:Prediction}. The later line of work was pioneered by~\citet{Daskalakis11:Near}, and has been thereafter extended along several lines~\citep{Rakhlin13:Online,Rakhlin13:Optimization,Syrgkanis15:Fast,Chen20:Hedging,Daskalakis21:Near,Daskalakis21:Fast,Piliouras21:Optimal}, incorporating partial or noisy information feedback~\citep{Foster16:Learning,Wei18:More,Hsieh22:No}, and more recently, general Markov games~\citep{Erez22:Regret,Zhang22:Policy}.

==> text/preliminaries.tex <==
\section{Preliminaries}
\label{section:prel}

In this section, we introduce our notation and basic background on online optimization and learning in games. For a more comprehensive treatement on those subjects, we refer to~~\citep{Shalev-Shwartz12:Online} and~\citep{Cesa-Bianchi06:Prediction}, respectively.

\paragraph{Notation} We denote by $\N = \{1, 2, \dots, \}$ the set of natural numbers. We use the variable $i$ with a subscript to index a player, and $t$ with a superscript to indicate the (discrete) time. To access the $\ind$-th coordinate of a $d$-dimensional vector $\vx \in \R^d$, for some $\ind \in \range{d} \defeq \{1, 2, \dots, d\}$,
we use the symbol $\vx[\ind]$.

\paragraph{Online learning and regret} Let $\cX \subseteq [0,1]^d$ be a nonempty convex and compact set, for $d \in \N$. In the framework of online learning, a learner (or a player)---denoted by $\regdep$---interacts with the environment at every time $t \in \N$ via the following subroutines.

\begin{itemize}
    \item $\regdep.\nextstrat()$: The learner outputs its next strategy $\vx^{(t)} \in \cX$ based on its internal state; and
    \item $\regdep.\obsutil(\ut^{(t)})$: The learner receives a feedback from the environment in the form of a utility vector $\ut^{(t)} \in\R^{d}$. 
\end{itemize}
The canonical measure of performance in online learning is the notion of \emph{regret}, denoted by $\reg^T$, which is defined, for a fixed time horizon $T \in \N$, as
\begin{equation}
    \label{eq:extreg}
    \max_{\vxstar \in \cX} \left\{ \sum_{t=1}^T \langle \vxstar, \ut^{(t)} \rangle \right\} - \sum_{t=1}^T \langle \vx^{(t)}, \ut^{(t)} \rangle.
\end{equation}
In words, the performance of the learner is compared to the performance of playing an optimal \emph{fixed strategy} in hindsight. We will say that the agent has \emph{no-regret} if $\reg^T = o(T)$, under \emph{any} sequence of observed utilities.

A much more general performance metric is \emph{$\Phi$ regret}, parameterized by a set of \emph{transformations} $\Phi : \cX \to \cX$. Namely, $\Phi$-regret for a time horizon $T \in \N$, denoted by $\reg^T_{\Phi}$, is defined as
%
\begin{equation}
    \label{eq:phireg}
    \sup_{\phistar \in \Phi} \left\{ \sum_{t=1}^T \langle \phistar(\vx^{(t)}), \ut^{(t)} \rangle \right\} - \sum_{t=1}^T \langle \vx^{(t)}, \ut^{(t)} \rangle.
\end{equation}
External regret~\eqref{eq:extreg} is simply a special case of~\eqref{eq:phireg} when $\Phi$ includes all possible \emph{constant transformations}, but $\Phi$ regret can be much more expressive. A celebrated game-theoretic motivation for $\Phi$ regret stems from the fact that when all players employ suitable $\Phi$-regret minimizers, the dynamics converge to different notions of \emph{correlated equilibria}, well-beyond \emph{coarse correlated equilibria}~\citep{Foster97:Calibrated,Stoltz07:Learning,Hart00:Simple,Celli20:No-Regret}.

\paragraph{From external to $\Phi$ regret} As it turns out, there is a general template for minimizing $\Phi$-regret due to~\citet{Gordon08:No}. In particular, their algorithm assumes access to the following.

\begin{enumerate}
    \item \label{item:phiexternal} A \emph{no-external-regret} $\regdep_\Phi$ operating \emph{over the set of transformations} $\Phi$; and
    \item A \emph{fixed point oracle} $\fp(\phi)$ that, for any $\phi \in \Phi$, computes a fixed point $\vx \in \cX$, under the assumption that such a point indeed exists.\label{item:fp}
\end{enumerate}
%
Based on those ingredients, \citet{Gordon08:No} were able to construct a regret minimization algorithm $\regdep$ with sublinear $\Phi$ regret, as illustrated in \Cref{algo:Gordon}. Specifically, $\regdep$ determines its next strategy by first obtaining the strategy $\phi^{(t)}$ of $\regdep_{\Phi}$ (\Cref{line:stratphi}), and then outputing any fixed point of $\phi^{(t)}$ (\Cref{line:fp}). Then, upon receiving the utility vector $\ut^{(t)} \in \R^d$, $\regdep$ forwards as input to $\regdep_{\Phi}$ the utility function $\phi \mapsto \langle \ut^{(t)}, \phi(\vx^{(t)}) \rangle$. We will assume that $\Phi$ contains \emph{linear transformations}, in which case that utility can be represented as $\Ut^{(t)} \defeq \ut^{(t)} \otimes \vx^{(t)}$ (\Cref{line:outer}), where $\otimes$ denotes the outer product of the two vectors. This algorithm enjoys the following guarantee.

\begin{algorithm}[!ht]
    \SetAlgoLined
    \SetInd{2.3mm}{2.3mm}
    \DontPrintSemicolon
    \KwData{An external regret minimizer $\regdep_{\Phi}$ for $\Phi$}    
        \BlankLine{}
        \Fn{$\nextstrat()$}{
            $\phi^{(t)} \leftarrow \regdep_{\Phi}.\nextstrat()$ \label{line:stratphi} \\
            $\vec{x}^{(t)} \leftarrow \fp(\phi^{(t)})$ \label{line:fp} \\
            \textbf{return} $\vec{x}^{(t)}$
        }
        \Hline{}
        \Fn{$\obsutil(\ut^{(t)})$}{
            Construct the utility $\Ut^{(t)} \leftarrow \ut^{(t)} \otimes\vec{x}^{(t)}$ \label{line:outer} \\
            $\regdep_{\Phi}.\obsutil(\Ut^{(t)})$
        }
    \caption{$\Phi$-Regret Minimizer~\citep{Gordon08:No}}
    \label{algo:Gordon}
\end{algorithm}

\begin{theorem}[\citep{Gordon08:No}]
    \label{theorem:gordon}
    Let $\reg^T$ be the external regret of $\regdep_{\Phi}$, and $\reg_{\Phi}^T$ be the $\Phi$-regret of $\regdep$. Then, for any $T \in \N$,
    \begin{equation*}
        \reg^T = \reg_{\Phi}^T.
    \end{equation*}
\end{theorem}

\paragraph{No-Regret learning in games} 
The main focus of our paper is about the behavior of no-regret learning dynamics when employed by all players in $n$-player games. More precisely, we will assume that the strategy set of each player $i \in \range{n}$ is a nonempty convex and compact set $\cX_i$. Further, the utility function $u_i : \bigtimes_{i'=1}^n \cX_{i'} \to \R$ of each player $i \in \range{n}$ is assumed to be multilinear, so that for any $\vx_{-i}$, $u_i(\vx) \defeq \langle \vx_i, \ut_i (\vx_{-i}) \rangle$; our results immediately apply to games with concave utilities~\citep{Rosen65:Existence,Hsieh21:Adaptive}. We will also let $L \geq 1$ be a Lipschitz constant of the utilities, in the sense that for any player $i \in \range{n}$ and $\vx_{-i}, \vx'_{-i} \in \bigtimes_{i' \neq i} \cX_{i'}$,
\begin{equation}
    \label{eq:Lip}
    \| \ut_i(\vx_{-i}) - \ut_i(\vx_{-i}') \|_\infty \leq L \|\vx_{-i} - \vx_{-i}'\|_1.
\end{equation}
%
In this context, learning procedures work as follows. At every iteration $t \in \N$ each player $i \in \range{n}$ commits to a strategy $\vx_i^{(t)} \in \cX_i$, and subsequently receives as feedback the utility corresponding to the other players' strategies at time $t$: $\ut_i^{(t)} \defeq \ut_i(\vx_{-i}^{(t)})$. It is assumed that players use no-regret learning algorithms to adapt to the behavior of the other players, leading to \emph{uncoupled} learning dynamics, in the sense that players do not use information about other players' utilities~\citep{Hart00:Simple,Daskalakis11:Near}. For convenience, and without any loss, we assume that $\| \ut_i^{(t)}\|_\infty \leq 1$, for $i \in \range{n}$ and $t \in \N$.

==> text/result.tex <==
\section{Main Result}
\label{sec:result}

In this section, we formalize our main result in \Cref{theorem:main}, the informal version of which was presented earlier in \Cref{theorem:informal}. Before we proceed with our key assumptions, let us first make some further conventions. We will assume that each linear transformation $\phi \in \Phi$ will be represented via its unique vector representation $\vX \subseteq [0,1]^{\phidim}$, for some $\phidim \in \N$; with a slight of notation, we will write $\vX \in \Phi$. Also, we will let $\xnorm \defeq \max_{\vx \in \cX} \|\vx\|_1 \geq 1$ and $\phinorm \defeq \max_{\vX \in \Phi} \|\vX\|_1 \geq 1$.

When treating the problem of $\Phi$-regret minimization from a computational standpoint, further assumptions have to be imposed on the set $\Phi$ to ensure that the problem is---at the very least---computationally interesting. In this context, each of our assumptions below relates to one of the premises of the construction of~\citet{Gordon08:No} (\Cref{item:phiexternal,item:fp}). In particular, we recall that the first ingredient (\Cref{item:phiexternal}) requires an external regret minimizer operating over the set $\Phi$. Naturally, when $\Phi$ is high-dimensional, this assumption is computationally reasonably when $\Phi$ is sufficiently structured. For our purposes, we will assume the existence of an efficient algorithm $\Pi_{\Tilde{\vW}}(\Tilde{\Ut}) $ for computing ``local'' proximal points:
\begin{equation}
    \label{eq:proxoracle}
    \argmin_{\Tilde{\vX} \in \Tilde{\Phi}} \left\{ \langle \Tilde{\vX}, \Tilde{\Ut} \rangle + \frac{1}{2} \| \Tilde{\vX} - \Tilde{\vW}\|^2_{\Tilde{\vW}} \right\},
\end{equation}
for any $\Tilde{\vW} \in \R^{\phidim+1}_{> 0}$ and $\Tilde{\Ut} \in \R^{\phidim+1}$, where 
\begin{equation}
    \label{eq:phitil}
\Tilde{\Phi} \defeq \left\{ (\lambda, \lambda \Phi) : \lambda \in [0,1] \right\},
\end{equation}
and
\begin{equation*}
    \| \Tilde{\vX} - \Tilde{\vW}\|^2_{\Tilde{\vW}} \defeq \sum_{\edg \in \range{D+1}} \left( \frac{\Tilde{\vX}[\edg] - \Tilde{\vW}[\edg]}{\Tilde{\vW}[\edg]} \right)^2.
\end{equation*}
%
This brings us to our first key assumption:

\begin{assumption}
    \label{assumption:efficiency}
    For any $\Tilde{\vW} \in \R^{\phidim+1}_{> 0}$ and $\Tilde{\Ut} \in \R^{\phidim+1}$ we can efficiently compute the local proximal point~\eqref{eq:proxoracle}.
\end{assumption}

Our second assumption is about the behavior of the fixed points of $\Phi$ (\Cref{item:fp}). $\Phi$ regret can, in general, capture complex and computationally intractable fixed point operations~\citep{Hazan07:Computational}. So, we have to impose some structure on the behavior of the fixed points. The key insight is to allow arbitrary rational functions with positive coefficients:

\begin{assumption}
    \label{assumption:rational}
For any function $\phi \in \Phi$, uniquely represented by $\vX$, the following properties hold.
\begin{enumerate}
    \item There exists $\vxstar \in \cX$ such that $\phi(\vxstar) = \vxstar$, and such a fixed point can be efficiently computed. Further, if $\vX$ is such that $\vX[\edg] \neq 0$, for all $\edg \in \range{\phidim}$, then the fixed point must be unique; and \label{item:unique}
    \item\label{item:rational} If $\vX[\edg] \neq 0$, for all $\edg \in \range{\phidim}$, then for any $\ind \in \range{d}$,
    \begin{equation*}
        \vxstar [\ind] = \sum_{k=1}^m \frac{p_{r, k}(\vX)}{q_{r, k}(\vX)},
    \end{equation*}
    for some multivariate polynomials $p_{r, k}, q_{r, k}$ with positive coefficients and maximum degree $\deg \in \N$.
\end{enumerate}
\end{assumption}
To be more concrete, let us relate this assumption with the construction of~\citet{Blum07:From} for minimizing \emph{swap regret}, an instance of $\Phi$ regret in normal-form games. In their construction, $\Phi$ corresponds to the set of all stochastic matrices. In that context, \Cref{item:unique} postulates uniqueness of the stationary distribution away from the singularity boundary---a well-known implication of the ergodicity of the associated Markov chain. Further, \Cref{item:rational} is a consequence of the \emph{Markov chain tree theorem}~\citep{Anantharam89:A}. 

While requiring only positive coefficients in \Cref{item:rational} may seem restrictive at first glance, in \Cref{prop:poscoeffs,prop:poscoeffs-tree} we show that it comes without any loss if the strategy set has a ``hierarchical structure.'' In particular, we give a procedure that gradually eliminates the negative monomials, without altering the degree of the underlying polynomial; this can be used, for example, to bypass the use of the Markov chain tree theorem to establish~\Cref{item:rational}.

We are now ready to state the formal version of \Cref{theorem:informal}.

\begin{theorem}
    \label{theorem:main}
    Consider a set of deviations $\Phi$ such that \Cref{assumption:rational,assumption:efficiency} hold. Then, there exist efficient and uncoupled learning dynamics that, when employed by all players for $T$ repetitions, the $\Phi_i$-regret of each player $i \in \range{n}$ is bounded as
    \begin{equation*}
        \reg_{\Phi_i}^T \leq (4096 L n (D+1) \phinorm \xnorm \deg) \log T.
    \end{equation*}
\end{theorem}

This establishes near-optimal regret when \emph{all} players employ specific learning dynamics. Further, it is also immediate to obtain at the same time optimal $O(\sqrt{T})$ regret in the \emph{adversarial setting}, where the other players act so as to maximize the player's regret.


\section{The Construction}

In this section, we provide and analyze the learning dynamics that establish \Cref{theorem:main}. Besides~\Cref{algo:Gordon}, the key algorithmic ingredient is \algoshort, a recent algorithm by~\citet{Farina22:Near}. \algoshort is an instance of \emph{optimistic follow the regularized leader (OFTRL)}~\citep{Syrgkanis15:Fast} with logarithmic regularization, operating over an appropriately lifted space. 

For our purposes, we will use \algoshort to construct $\regdep_{\Phi}$, the regret minimizer over the set of transformations $\Phi$. In particular, if $\Tilde{\Phi}$ is defined as in~\eqref{eq:phitil}, \algoshort updates $\Tilde{\vX}^{(t)} = (\lambda^{(t)}, \vY^{(t)}) \in \Tilde{\Phi}$, for a time $t \in \N$, as
%
\begin{equation}
    \label{eq:lrl}
    \argmax_{\Tilde{\vX} \in \Tilde{\Phi}} \left\{ \eta \left\langle \vS^{(t-1)}, \Tilde{\vX} \right\rangle + \!\!\!\!\!\sum_{\edg \in \range{\phidim + 1}}  \!\!\!\!\!\log \Tilde{\vX}[\edg] \right\},
\end{equation}
where we let $\vS^{(t-1)} \defeq \tilde{\Ut}^{(t-1)} + \sum_{\tau=1}^{t-1} \Tilde{\Ut}^{(\tau)}$; $\Tilde{\Ut}^{(t)} \defeq (- \langle  \vX^{(t)}, \Ut^{(t)} \rangle, \Ut^{(t)})$, and $\eta > 0$ is the learning rate. The first key property of \algoshort is that it can be efficiently implemented on $\Phi$---with $O(\log \log T)$ iteration complexity---if \Cref{assumption:efficiency} holds.
%
\begin{proposition}
    If \Cref{assumption:efficiency} holds, \algoshort~\eqref{eq:lrl} can be efficiently implemented on the set $\Phi$.
\end{proposition}

Moreover, \algoshort guarantees the following refined \emph{RVU} (see \citep{Syrgkanis15:Fast}) bound.

\begin{restatable}{proposition}{rvuoriginal}
    \label{proposition:rvu-original}
    For any learning rate $\eta \leq \frac{1}{256 \phinorm}$ and $T \geq 2$, $\max\{0, \reg^T_{\Phi} \}$ can be upper bounded by
    \begin{align*}
        2 \frac{(D+1) \log T}{\eta} &+ 16 \eta \phinorm^2 \sum_{t=1}^{T-1} \|\Ut^{(t+1)} - \Ut^{(t)} \|_\infty^2 \\
        &- \frac{1}{32\eta} \sum_{t=1}^{T-1} \left\| \begin{pmatrix}
            \lambda^{(t+1)} \\
            \vY^{(t+1}
        \end{pmatrix} -
        \begin{pmatrix}
            \lambda^{(t)} \\
            \vY^{(t}
        \end{pmatrix}
        \right\|^2_{t}.
    \end{align*}
\end{restatable}
This is a slight modification of~\citep[Proposition 2 and Corollary 1]{Farina22:Near}, leveraging \Cref{theorem:gordon}. Now the main goal is to cast \Cref{proposition:rvu-original} in terms of the strategies $\vx^{(t)}$ and the utilities $\ut^{(t)}$ associated with the player. The first step is to use the following relation between the multiplicative deviations in the original space $\Phi$ and the lifted space $\Tilde{\Phi}$, which is a consequence of using the logarithmic regularizer in~\eqref{eq:lrl}.

\begin{restatable}{lemma}{gammaterm}
    \label{lemma:mul-dev}
    For $t \in \N$ and learning rate $\eta \leq \frac{1}{50 \phinorm}$,
    \begin{align*}
        \max_{\edg \in \range{D}} \left| 1 - \frac{\vX^{(t)}[\edg]}{\vX^{(t-1)}[\edg]} \right| &\leq 4 \left\| \begin{pmatrix}
            \lambda^{(t)} \\
            \vY^{(t)}
        \end{pmatrix} - 
        \begin{pmatrix}
            \lambda^{(t-1)} \\
            \vY^{(t-1)}
        \end{pmatrix}
        \right\|_{t, \infty} \\
        &\leq 100 \eta \phinorm.
    \end{align*}
\end{restatable}

The next key step is to bound the deviation of the strategies $\vx^{(t)}$ in terms of the deviation of the transformations $\vX^{(t)}$. This is where \Cref{assumption:rational} turns out to be crucial, enabling the following key lemma.

\begin{restatable}{lemma}{gamma}
    \label{lemma:gamma}
Suppose that $\Phi$ satisfies \Cref{assumption:rational}. If $\eta \leq \frac{1}{256\deg \phinorm}$, then for any $t \in \N$,
\begin{equation*}
    \| \vx^{(t+1)} - \vx^{(t)} \|_1 \leq (4 \xnorm \deg) \max_{\edg \in \range{D}} \left| 1 - \frac{\vX^{(t)}[\edg]}{\vX^{(t-1)}[\edg]} \right|.
\end{equation*}
\end{restatable}
Importantly, the number of rational functions---parameter $m$ in~\Cref{item:rational}---or the number of monomials in each polynomial do not affect the bound. Also, it is possible to improve \Cref{lemma:gamma} if the underlying polynomials have more structure than what imposed by~\Cref{assumption:rational}, but we opted for the more general conditions here, ultimately losing sharpness in some bounds. 

As a result, combining \Cref{lemma:mul-dev,lemma:gamma} with \Cref{proposition:rvu-original}, and using the structure of $\Ut^{(t)}$ (\Cref{line:outer}), we obtain the following RVU bound for the original space $\cX$.

\begin{restatable}{corollary}{rvu}
    \label{proposition:rvu-original}
    For any $\eta \leq \frac{1}{2^{10} \phinorm \xnorm \deg}$ and $T \geq 2$, $\max\{0, \reg^T_{\Phi} \}$ can be upper bounded as
    \begin{align*}
        2 \frac{(D+1) \log T}{\eta} &+ 32 \eta \phinorm^2 \sum_{t=1}^{T-1} \|\ut^{(t+1)} - \ut^{(t)} \|_\infty^2 \\
        &- \frac{1}{2^{14} \eta \xnorm^2 \deg^2} \sum_{t=1}^{T-1} \left\| \vx^{(t+1)} - \vx^{(t)}
        \right\|^2_{1}.
    \end{align*}
\end{restatable}
With this RVU bound at hand, the proof of \Cref{theorem:main} follows the argument of~\citet{Anagnostides22:Uncoupled}.

\section{Applications in Extensive-Form Games}

In this section, we provide two main applications of our general framework (\Cref{theorem:main}) in extensive-form games (EFGs), leading to the first near-optimal learning dynamics for extensive-form correlated and coarse correlated equilibria in EFGs (\Cref{cor:trigger,cor:ctrigger}). First, let us introduce some basic background on EFGs.

\subsection{Background on EFGs}

An extensive-form game is played on a rooted and directed tree with node-set $\cH$. Every \emph{decision (non-terminal) node} $h \in \cH$ is uniquely associated with a player who selects an action from a finite and nonempty set $\cA_h$. By convention, the set of players includes a fictitious ``chance'' player $c$ that acts according to a fixed distribution. The set of \emph{leaves (terminal) nodes} $\cZ \subseteq \cH$ correspond to different outcomes of the game. Once the game reaches a terminal node $z \in \cZ$, every player $i \in \range{n}$ receives a payoff according to a utility function $u_i : \cZ \to [-1, 1]$. 

In an imperfect-information EFG, the decision nodes of each player $i \in \range{n}$ are partitioned into \emph{information sets} $\cJ_i$. For an information set $j \in \cJ_i$ and an action $a \in \cA_j$, we let $\sigma \defeq (j,a)$ be the \emph{sequence} of $i$'s actions encountered from the root of the tree until action $a$; we use the special symbol $\emptyseq$ to denote the \emph{empty sequence}. The set of $i$'s sequences is denoted by $\Sigma_i \defeq \{ (j,a) : j \in \cJ_i, a \in \cA_j \} \cup \{ \emptyset \}$; we also let $\Sigma_i^* \defeq \Sigma_i \setminus \{\emptyset\}$. We will write $\sigma_j$ to represent the \emph{parent sequence} of an information set $j \in \cA_j$; namely, the last sequence before reaching $j$, or $\emptyseq$ if $j$ is a \emph{root information set}.

\paragraph{Sequence-form strategies} The strategy of a player specifies a probability distribution for every information set encountered in the tree. Assuming \emph{perfect-recall}---players never forget acquired information---the strategy can be represented via the \emph{sequence-form strategy polytope} $\cQ_i \subseteq \R_{\geq 0}^{|\Sigma_i|}$, defined as follows.
%
\begin{equation*}
    \left\{ \vq_i : \vq_i[\emptyseq] = 1, \vq_i[\sigma_j] = \sum_{a \in \cA_j} \vq_i[(j,a)], \forall j \in \cJ_i \right\}.
\end{equation*}
Further, we let $\Pi_i \defeq \cQ_i \cap \{0,1\}^{|\Sigma_i|}$ be the \emph{deterministic} sequence-form strategies. Analogously, one can define the sequence-form polytope $\cQ_j$ rooted at $j$. In accordance to our notation, we use $\qnorm$ to denote the maximum $\ell_1$-norm of a $\vq_i \in \cQ_i$. Finally, we let $\depth_i$ denote the depth of $i$'s subtree.

\paragraph{Trigger deviations and EFCE}

To formalize the connection between EFCE and the framework of Phi-regret, we first introduce \emph{trigger deviation functions}.

\begin{definition}[\citep{Farina21:Simple}]
    \label{def:trigdev}
    A trigger deviation function with respect to a trigger sequence $\hat{\sigma} = (j,a) \in \Sigma_i^*$ and a continuation strategy $\hat{\vec{\pi}}_i \in \Pi_j$ is any linear mapping $f : \R^{|\Sigma_i|} \to \R^{|\Sigma_i|}$ such that
    \begin{itemize}
        \item $f(\vec{\pi}_i) = \vec{\pi}_i$ for all $\vec{\pi}_i \in \Pi_i$ such that $\vec{\pi}_i[\hat{\sigma}] = 0$; \item Otherwise, for all $\vec{\pi}_i \in \Pi_i$,
        \begin{equation*}
            f(\vec{\pi}_i)[\sigma] =
            \begin{cases}
             \vec{\pi}_i[\sigma] \quad  \text{if } \sigma \not\succeq j, \\
             \hat{\vec{\pi}}_i[\sigma] \quad \text{if } \sigma \succeq j.
        \end{cases}
        \end{equation*}
    \end{itemize}
\end{definition}

We will denote by $\Psi_i$ the convex hull of all trigger deviation functions---over all trigger sequences and (deterministic) continuation strategies; $\Psi_i$-regret will be referred to as \emph{trigger regret}. In an \emph{extensive-form correlated equilibrium}~\citep{Stengel08:Extensive} no trigger deviation can improve the expected utility of that player, leading to the following connection.

\begin{proposition}[\citep{Farina21:Simple}]
    \label{prop:deg-efcce}
    If each player $i$ incurs trigger regret $\reg_{\Psi_i}^T$ after $T$ repetitions, the average product distribution of play is a $\frac{1}{T} \max_{i \in \range{n}} \Psi_i$-approximate EFCE.
\end{proposition}

Extensive-form \emph{coarse} correlated equilibria (EFCCE)~\citep{Farina20:Coarse} are defined analogously based on \emph{coarse trigger deviations} $\Tilde{\Psi}_i$; the difference is that in EFCCE the player gets to decide whether to follow the recommendation \emph{before} actually seeing the recommendation at that information set.

\subsection{EFCCE}

We will first apply our framework to EFFCE. We note that some entries in the (coarse) trigger deviation functions are always constant; those coordinates do not cumulate any regret, and are removed before employing~\algoshort. Now regarding efficiently implementation of \algoshort (\Cref{assumption:efficiency}), we show the following.

\begin{proposition}
    \label{prop:efce-eff}
    Trigger deviations $\Psi_i$ and coarse trigger deviations $\Tilde{\Psi}_i$ satisfy~\Cref{assumption:efficiency}.
\end{proposition}

This extends prior work by efficiently implementing a proximal oracle for the convex hull of sequence-form polytopes. So, let us focus on \Cref{assumption:rational}: the existence of a rational fixed-point characterization in the sense of~\Cref{item:rational}. To do so, we leverage a closed-form characterization for EFCCE~\citep{Anagnostides22:Faster}, leading to the following result.

\begin{restatable}{proposition}{efccerational}
    \label{proposition:efcce-rational}
    The fixed points of any coarse trigger deviation function $\phi_i \in \Tilde{\Psi}_i$ satisfy \Cref{assumption:rational} with $\deg = O(\depth_i)$.
\end{restatable}

As a result, using that $\|\Tilde{\Psi}_i \|_1, \|\Psi_i\|_1 = O(\|\cQ_i\|_1)$, as well as the fact that EFGs are $|\cZ|$-Lipschitz~\citep{Anagnostides22:Faster}, we arrive at the following guarantee.

\begin{corollary}
    \label{cor:ctrigger}
    If all players employ \Cref{algo:Gordon} instantiated with \algoshort for $T$ repetitions, the coarse trigger regret of each player $i \in \range{n}$ will be bounded as
    \begin{equation*}
        \reg^T_{\Tilde{\Psi}_i} \leq  C n |\Sigma|^2 \|\cQ\|_1^2 \|\cZ\| \depth \log T,
    \end{equation*}
    for a universal constant $C > 0$.
\end{corollary}

\subsection{EFCE}

Next, we show that the set $\Psi_i$ also satisfies \Cref{assumption:efficiency} with small maximum degree. Unlike EFCCE, the fixed points associated with EFCE are much more involved, requiring gradually computing stationary distributions of Markov chains along paths of the tree. Nevertheless, using a refined characterization of its stationary distribution~\citep{Anagnostides22:Faster} as our inductive step, we establish the following guarantee.

\begin{restatable}{proposition}{efcerational}
    \label{prop:deg-efce}
    The fixed points of any trigger deviation function $\phi_i \in \Psi_i$ satisfy \Cref{assumption:rational} with $\deg = O(\depth_i |\cA_i|)$, where $|\cA_i| \defeq \max_{j \in \cJ_i} |\cA_j|$.
\end{restatable}

As a result, our bound on the maximum degree for EFCE is only a factor $|\cA_i|$ away compared to EFCCE (\Cref{prop:deg-efcce}). Combining with \Cref{theorem:main}, we conclude the following.

\begin{corollary}
    \label{cor:trigger}
    If all players employ \Cref{algo:Gordon} instantiated with \algoshort for $T$ repetitions, the trigger regret of each player $i \in \range{n}$ will be bounded as
    \begin{equation*}
        \reg^T_{\Psi_i} \leq C n |\Sigma|^2 \|\cQ\|_1^2 \|\cZ\| |\cA| \depth \log T,
    \end{equation*}
    for a universal constant $C > 0$.
\end{corollary}
